Joint Chance Constrained Safe-Optimal Control

We consider the finite-time optimal control of stochastic systems subject to a probabilistic constraint on the trajectories' safety. Such formulations are known as joint chance constrained optimal control problems. The common practice is to jointly minimise the expected cost of all trajectories, safe and unsafe. This leads to policies which invite constraint violations to exploit low-cost unsafe trajectories. When constraints represent states of critical failure, such behaviour is undesirable. We demonstrate that this behaviour can be overcome by only minimizing the expected cost of safe trajectories. The underlying rationale follows a practical intuition: In many applications, the cost incurred by unsafe trajectories is irrelevant (e.g., the battery usage of a crashed quadcopter), and one is usually interested in minimizing the cost of trajectories that are safe. We show that this problem can be cast as a constrained Markov Decision Process over an augmented state space. This allows solving it via dynamic programming. We derive bounds on the policies' safety under errors resulting from gridding approximations when the system's state space is continuous. Finally, we empirically compare dynamic programming as well as reinforcement learning solutions on a simulated 2D unicycle system in cluttered reach-avoid environments.

==> data_pareto_jcc_classic.tex <==
Safety SafeCost UnsafeCost AllCost
0.0000 0.0000 0.0000 0.0000
0.0180 16.0370 0.3333 0.6160
0.5670 16.3310 0.9045 9.6513
0.5810 16.3448 0.8329 9.8453
0.5960 16.2584 0.7591 9.9967
0.6080 16.3761 1.0119 10.3533
0.6200 16.3516 0.8298 10.4533
0.6300 16.3556 0.8559 10.6207
0.6400 16.2583 0.6148 10.6267
0.6520 16.3006 0.7988 10.9060
0.9710 16.4638 9.8966 16.2733

==> data_pareto_jcc_safe.tex <==
Safety SafeCost UnsafeCost AllCost
0.0000 0.0000 0.0000 0.0000
0.0240 10.6389 3.1462 3.3260
0.0640 10.9688 3.6332 4.1027
0.0890 11.1723 4.0465 4.6807
0.1200 11.1000 4.0015 4.8533
0.1680 11.3373 4.6482 5.7720
0.2040 11.3954 4.5921 5.9800
0.2710 11.4182 4.8134 6.6033
0.3070 11.4213 5.0548 7.0093
0.3350 11.4836 5.3459 7.4020
0.3670 11.5758 5.5234 7.7447
0.3980 11.9983 6.2049 8.5107
0.4150 12.1791 6.7014 8.9747
0.4290 12.2556 6.8330 9.1593
0.4430 12.2897 6.6302 9.1373
0.4530 12.5085 6.8635 9.4207
0.4630 12.2196 6.8200 9.3200
0.4740 12.6160 6.6426 9.4740
0.4870 12.7632 6.8233 9.7160
0.5470 13.2291 6.8572 10.3427
0.6020 14.3333 6.8559 11.3573
0.6220 14.7181 6.8254 11.7347
0.7800 15.9188 7.0636 13.9707
0.9090 16.6370 7.4249 15.7987
0.9530 17.0035 8.6879 16.6127
0.9640 17.0090 9.7407 16.7473
0.9740 17.1020 8.3846 16.8753
